A Synergistic Compilation Workflow for Tackling Crosstalk in Quantum Machines

Near-term quantum systems tend to be noisy. Crosstalk noise has been recognized as one of several major types of noises in superconducting Noisy Intermediate-Scale Quantum (NISQ) devices. Crosstalk arises from the concurrent execution of two-qubit gates on nearby qubits, such as \texttt{CX}. It might significantly raise the error rate of gates in comparison to running them individually. Crosstalk can be mitigated through scheduling or hardware machine tuning. Prior scientific studies, however, manage crosstalk at a really late phase in the compilation process, usually after hardware mapping is done. It may miss great opportunities of optimizing algorithm logic, routing, and crosstalk at the same time. In this paper, we push the envelope by considering all these factors simultaneously at the very early compilation stage. We propose a crosstalk-aware quantum program compilation framework called CQC that can enhance crosstalk mitigation while achieving satisfactory circuit depth. Moreover, we identify opportunities for translation from intermediate representation to the circuit for application-specific crosstalk mitigation, for instance, the \texttt{CX} ladder construction in variational quantum eigensolvers (VQE). Evaluations through simulation and on real IBM-Q devices show that our framework can significantly reduce the error rate by up to 6$\times$, with only $\sim$60\% circuit depth compared to state-of-the-art gate scheduling approaches. In particular, for VQE, we demonstrate 49\% circuit depth reduction with 9.6\% fidelity improvement over prior art on the H4 molecule using IBMQ Guadalupe. Our CQC framework will be released on GitHub.

==> case.tex <==
\subsection{Application Opportunities}
\label{sec:VQE}
In this section, we will talk about the more opportunity we found in specific applications using VQE as an example. Here we take the VQE as our case study since VQE is really important in near-term quantum algorithms. We can further optimize the VQE based on our existing compiler framework. Through our improvement, VQE for molecular research can be much simpler or trained faster. Our optimization workflow is shown in Figure~~\ref{fig:vqeframe}, we find the optimization opportunity lies in the three parts we will discuss all the components in detail.
\begin{enumerate}
    \item Hamiltonian Generation and decoding Pauli string: we can generate different Hamiltonian and Pauli strings based on different molecule geomery/basis method/decoding method/excitation numbers, so by changing the parameter, we can generate the Pauli-string which has less depth and crosstalk.
    \item Crosstalk-aware
    circuit evaluation: We have multiple choices to generate different circuit patterns for each pauli strings, by inserting different swaps, we will have different circuit patterns, we want to define a cost function which can guide us choose the near-optimal circuit pattern which has less depth and crosstalk.
    \item Look-ahead optimization: To further seek the optimization choices, we take the next step circuit as a weight for our layout optimization, To move from the current Pauli string to next, we need to add necessary swaps to change the layout. However, different choices may lead to less swaps and less crosstalk. We can choose the current Pauli string circuit by using the look-ahead optimization.
\end{enumerate}
% 1) Hamiltonian Generation and decoding Pauli string: we can generate different Hamiltonian and Pauli strings based on different molecule geomery/basis method/decoding method/excitation numbers, so by changing the parameter, we can generate the Pauli-string which has less depth and crosstalk. 2) Crosstalk-aware
% circuit evaluation: We have multiple choices to generate different circuit patterns for each pauli strings, by inserting different swaps, we will have different circuit patterns, we want to define a cost function which can guide us choose the near-optimal circuit pattern which has less depth and crosstalk. 3) Look-ahead optimization: To further seek the optimization choices, we take the next step circuit as a weight for our layout optimization, To move from the current Pauli string to next, we need to add necessary swaps to change the layout. However, different choices may lead to less swaps and less crosstalk. We can choose the current Pauli string circuit by using the look-ahead optimization.

\begin{figure}[htp]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/VQEframework.pdf}
  \caption{The VQE workflow showcasing application-specific optimization.}
  \label{fig:vqeframe}
\end{figure}






\subsubsection{Hamiltonian Generation and decoding Pauli string}
To show our optimization in VQE application, we first need to generate the hamiltonian function which is decided by the following terms:
\begin{enumerate}
    \item Molecule: choose the atoms in the molecule from the simplest "H" to "Li, Be" and so on, different molecule will generate different \textit{Pauli strings}, for instance  "Li-2" will generate $10\times$ more terms compared with "H-2" in the same geometry and basis.
    \item Geometry: The atoms in the molecule can be represented in different geometry structure which also affect the Hamiltonian function, like square and linear also lead to different number of \textit{Pauli strings}.
    \item Basis: We use pyscf \cite{sun2020recent} to generate hamiltonian function, which has different GTO basis options such as "sto-3g", "631++". 
\end{enumerate}

\begin{figure}[htp]
  \centering
  \includegraphics[width=0.8\linewidth]{fig/VQE_geomery.pdf}
  \caption{The transformation for different molecular geometry}
  \label{fig:vqegeo}
\end{figure}
By changing the geometry for the same molecular, we have different number of Pauli Strings which show in figure \ref{fig:vqegeo} 



To better illustrate this process, we will show the hydrogen molecule in the STO-3G basis with the Jordan-Wigner encoding\cite{mcardle2020quantum}. It starts with a Hamiltonian function shown as below:
\begin{equation}
\begin{split}
    H = H_1 + H_2 = \sum_{p,q}h_{pq}a_{p}^{\dagger}a_{q} + \frac{1}{2}h_{pqrs}a_{p}^{\dagger}a_{q}^{\dagger}a_{r}a_{s}
\end{split}
\label{formula:ham}
\end{equation}
where $a_{p}^{\dagger}$is the fermionic creation operator for fermionic mode (spin orbital) p
and $a_{p}$ is the fermionic annihilation operator for fermionic mode (spin orbital) 
Then for example, for hydrogen molecule in the STO-3G basis, it will finally become the Pauli Strings listed below (we omit some details here and will provide in appendix):
\begin{equation}
\begin{split}
H &=h_{00} a_{0}^{\dagger} a_{0}+h_{11} a_{1}^{\dagger} a_{1}+h_{22} a_{2}^{\dagger} a_{2}+h_{33} a_{3}^{\dagger} a_{3} \\
&+h_{0110} a_{0}^{\dagger} a_{1}^{\dagger} a_{1} a_{0}+h_{2332} a_{2}^{\dagger} a_{3}^{\dagger} a_{3} a_{2}+h_{0330} a_{0}^{\dagger} a_{3}^{\dagger} a_{3} a_{0} \\
&+h_{1221} a_{1}^{\dagger} a_{2}^{\dagger} a_{2} a_{1}+\left(h_{0220}-h_{0202}\right) a_{0}^{\dagger} a_{2}^{\dagger} a_{2} a_{0} \\
&+\left(h_{1331}-h_{1313}\right) a_{1}^{\dagger} a_{3}^{\dagger} a_{3} a_{1}\\&+h_{0132}\left(a_{0}^{\dagger} a_{1}^{\dagger} a_{3} a_{2}+a_{2}^{\dagger} a_{3}^{\dagger} a_{1} a_{0}\right) \\
&+h_{0312}\left(a_{0}^{\dagger} a_{3}^{\dagger} a_{1} a_{2}+a_{2}^{\dagger} a_{1}^{\dagger} a_{3} a_{0}\right)
\end{split}
\label{formula:decoding}
\end{equation}
Then we will use Jordan-Wigner encoding to encode this formula based on rules below:
\begin{equation}
\begin{aligned}
&a_{j}^{\dagger}: Z_{0} \otimes \cdots \otimes Z_{j-1} \otimes \sigma_{j}^{+} \otimes I 
\end{aligned}
\end{equation}
where:
\begin{equation*}
\begin{aligned}
\sigma^{+}= & \frac{X-i Y}{2}=\frac{1}{2}\left(\left[\begin{array}{ll}
0 & 1 \\
1 & 0
\end{array}\right]-\right.
\left.i\left[\begin{array}{cc}
0 & -i \\
i & 0
\end{array}\right]\right)\\ = & \left[\begin{array}{ll}
0 & 0 \\
1 & 0
\end{array}\right]=|1\rangle\langle 0| 
\end{aligned}
\end{equation*}
so we have 
\begin{equation*}
\begin{aligned}
&\sigma^{+}|0\rangle=\left[\begin{array}{ll}
0 & 0 \\
1 & 0
\end{array}\right]\left[\begin{array}{l}
1 \\
0
\end{array}\right]=\left[\begin{array}{l}
0 \\
1
\end{array}\right]=|1\rangle \\
&\sigma^{+}|1\rangle=\left[\begin{array}{ll}
0 & 0 \\
1 & 0
\end{array}\right]\left[\begin{array}{l}
0 \\
1
\end{array}\right]=\left[\begin{array}{l}
0 \\
0
\end{array}\right] \\
&\{\left.\sigma^{+}, \sigma^{+}\right\}=0
\end{aligned}
\end{equation*}


Finally we can get the decoding result:
\begin{equation}
\begin{split}
     H=&\, h_{0} I+h_{1} Z_{0}+h_{2} Z_{1}+h_{3} Z_{2}+h_{4} Z_{3}+ h_{5} Z_{0} Z_{1}+h_{6} Z_{0} Z_{2} \\ & + h_{7} Z_{1} Z_{2}+h_{8} Z_{0} Z_{3} +  h_{9} Z_{1} Z_{3}+h_{10} Z_{2} Z_{3}+ h_{11} Y_{0} Y_{1} X_{2} X_{3} \\ & +h_{12} X_{0} Y_{1} Y_{2} X_{3} + h_{13} Y_{0} X_{1} X_{2} Y_{3}+h_{14} X_{0} X_{1} Y_{2} Y_{3} 
\end{split}
\label{formula:final}
\end{equation}

\subsubsection{Crosstalk-aware circuit evaluation}

Based on the decoding results, we can generate the \textit{Pauli strings}, we use the same sorting technique as Paulihedral\cite{li2022paulihedral}. However, for each \textit{Pauli strings},  the qubits on the \textit{Pauli strings} are not always connected, we need to connect different Pauli components by adding SWAPs. There are some flexibility here to adding SWAPs in order to make all components are connected which means we will generate different \textbf{Circuits}. So there are multiple ways to generate circuits from \textit{Pauli strings} which shown in Figure~~\ref{fig:vqeframe}. We want to choose the circuit which under the consideration of both crosstalk and depths, So we design a cost function which can quickly evaluate different \textbf{circuits} which takes depth and crosstalk into consideration. 

The cost function is shown in \ref{alg:vqe}, it will guide us to choose the optimal circuit pattern.   In-order to evaluate two terms of crosstalk and depth. We treat the crosstalk errors as additional depth since we can add barriers to aovid crosstalk, so crosstalk will lead to extra depths, so the total cost function will be $Cost = w1*crosstalk + depth +3*w2*SWAPs$, the SWAPs are the number of SWAPs to connected the different components.  And we choose the circuit which has the minimum cost value. "w" is the weight from 0 to 1, since two crosstalk happens at the same time only leads to one barrier. And same reason for SWAPs which can parallelism.
 \begin{algorithm}[!t]
      \caption{VQE cost function}
      \label{alg:vqe}
         \SetKwFunction{FMain}{calculate\_depths}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{Connected graph G}}{
        Convert(G) to Tree(T);,\\
        Root(T) = $Graph\_center$(G)\\
        \If{T has one branch}{
         return len(T)-1;
        }\Else {
             List = $ \emptyset $; crosstalk = 0;  \\
        
             \For{child\_node $c_i$ in T}{
                cur = calculate\_depths($c_i$) \\
                List.add(cur); \\
                % $maxd = max(maxd,calculate\_depths(c_i))$
    
            }
            sort(List);\\
            \For{$l_i$ in List}{
                \uIf{$i+1 < len(List)  and l_{i+1} == l_{i}$}{
                    $l_{i+1} = l_{i+1}+1$;
                }
    
            }
            \For{$l_i$ in List}{
            
                \uIf{i+1 < len(List)  and $|l_{i+1} - l_{i}| == 1 $}{
                    crosstalk = crosstalk + 1;
                }
    
            }
          
            depth = max(List)*2+1; \\
            crosstalk = crosstalk * 2;
        }
}

\end{algorithm} 
 

\begin{figure}[htp]
  \centering
  \includegraphics[width=1\linewidth]{fig/VQEcostfunc.pdf}
  \caption{VQE application study.}
  \label{fig:crosstalkvqe}
\end{figure}
To better illustrate We show an example in Figure~ \ref{fig:crosstalkvqe} to show how our cost function works to choose the best circuit pattern for us. Given the \textit{Pauli strings} as XXYZZXX, There are two components given current mapping , one is {0,1,2,3,4,6} another is {5}. We want to SWAP qubit 5 with qubit 7 to make all the qubits in the \textit{Pauli strings} are connected. However, there are several choices which shows in Figure~\ref{fig:crosstalkvqe} (c) . For instance, we can SWAP qubit 5 and 8 to generate \textbf{Circuit 1} . Also we can SWAP qubit 5 and 7 for \textbf{Circuit 2} or SWAP qubit 6 and 7 at the same time for \textbf{Circuit 3}. After we evaluate the pattern based on crosstalks and depths, based on our cost function we will choose pattern 1 and circuit 3 which has the same cost value.

After we choose the circuit pattern, we will generate the exponential gates with our crosstalk aware compiler talked before, it will generate the near-optimal circuit with consideration of crosstalk and depth.


\subsubsection{Look-ahead optimization}
We evaluate different circuit patterns based on each Pauli strings, but for different circuit patterns we need to insert swaps between Pauli strings. To carefully seek the optimization opportunity between the Pauli Strings, we use a look-ahead optimization strategy for next layer. To better illustrate this idea, we show an example in Figure\ref{fig:crosstalkvqe}(d), based on inserting swaps and evaluate circuit at current layer we have coverd in last paragraph, we find that we have two choices which has the same costs considering the circuit depth and crosstalk errors for current layer.

However if we use the look-ahead optimization method, we can further make a better choice depend on next layer Pauli String. By evaluating the circuit depth and crosstalk errors, we find that the Circuit 1 and 3 are equivalent which is shown in Figure \ref{fig:crosstalkvqe}(c). However, if we take the next Pauli String into consideration, now the qubit 6 is temporarily  not be used in the next Pauli String which is shown in Figure \ref{fig:crosstalkvqe}(d), then for circuit 3, the qubit 5 will be disconnected from qubit 0,1,2,3,4. So we need one more extra swaps. However for circuit 1 we can still find all qubits which will be used in the next Pauli String are connected and does not need any more extra swap. So based on look ahead optimization here, we will choose the circuit 1.

After we decide the circuit, we will generate them into the exponential gates for VQE. Based on our CQC, we will generate the circuit with promising depth and less crosstalk errors.


% \subsubsection{}
% Finally we will scheduling the gates to maximize the parallelism of the gates withouth leading to extra depths 
